OGLE-2017-BLG-0448Lb: A Low Mass-Ratio Wide-Orbit Microlensing Planet?

The gravitational microlensing technique is most sensitive to planets in a Jupiter-like orbit and has detected more than 200 planets. However, only a few wide-orbit ($s > 2$) microlensing planets have been discovered, where $s$ is the planet-to-host separation normalized to the angular Einstein ring radius, $\theta_{\rm E}$. Here we present the discovery and analysis of a strong candidate wide-orbit microlensing planet in the event, OGLE-2017-BLG-0448. The whole light curve exhibits long-term residuals to the static binary-lens single-source model, so we investigate the residuals by adding the microlensing parallax, microlensing xallarap, an additional lens, or an additional source. For the first time, we observe a complex degeneracy between all four effects. The wide-orbit models with $s \sim 2.5$ and a planet-to-host mass-ratio of $q \sim 10^{-4}$ are significantly preferred, but we cannot rule out the close models with $s \sim 0.35$ and $q \sim 10^{-3}$. A Bayesian analysis based on a Galactic model indicates that, despite the complicated degeneracy, the surviving wide-orbit models all contain a super-Earth-mass to Neptune-mass planet at a projected planet-host separation of $\sim 6$ au and the surviving close-orbit models all consist of a Jovian-mass planet at $\sim 1$ au. The host star is probably an M or K dwarf. We discuss the implications of this dimension-degeneracy disaster on microlensing light-curve analysis and its potential impact on statistical studies.

==> draft.tex <==

\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{Parameters of Models without Parallax for \eventf}
    \begin{tabular}{c|c c c|c}
    \hline
    \hline
    Parameters & Close A & Close B & Wide & 1L2S \\
    \hline
    $\chi^2$/dof & $1658.5/1653$ & $1685.2/1653$ & $1670.1/1653$ & $1684.6/1653$ \\
    \hline
    $t_{0,1}$ (${\rm HJD}^{\prime}$)  & $8024.377 \pm 0.019$ & $8024.371 \pm 0.018$ & $8024.369 \pm 0.019$ & $8024.369 \pm 0.020$ \\
    $t_{0,2}$ (${\rm HJD}^{\prime}$) & ...  & ... & ... & $8003.447 \pm 0.071$ \\
    $u_{0,1}$  & $0.0219 \pm 0.0014$ & $0.0246 \pm 0.0020$ & $0.0240 \pm 0.0013$ & $0.0245 \pm 0.0018$ \\
    $u_{0,2}$ & ... & ... & ... & $0.0000 \pm 0.0018$ \\
    $\te$ (days)  & $79.0 \pm 4.5$ & $71.1 \pm 5.1$ & $72.6 \pm 3.4$ & $70.7 \pm 4.6$ \\
    $\rho_1$ ($10^{-3}$) & $1.05_{-0.25}^{+0.40}$ & $2.04_{-0.51}^{+0.59}$ & $<1.5$ & ... \\
    $\rho_2$ ($10^{-3}$) & ... & ... & ... & $<7.0$ \\
    $q_{f,I} (10^{-3})$ & ... & ... & ... & $2.89 \pm 0.76$ \\
    $\alpha$ (rad)  & $0.0605 \pm 0.0037$ & $0.1060 \pm 0.0042$ & $3.2251 \pm 0.0014$ & ... \\
    $s$ & $0.8732 \pm 0.0064$ & $0.8623 \pm 0.0091$ & $1.1642 \pm 0.0095$ & ... \\
    $\log q$ & $-4.545 \pm 0.158$ & $-4.693 \pm 0.146$ & $-4.872 \pm 0.117$ & ... \\
    $I_{\rm S, KMTC}$ & $21.26 \pm 0.07$ & $21.14 \pm 0.08$ & $21.16 \pm 0.06$ & $21.19 \pm 0.08$ \\
    \hline
    \hline
    \end{tabular}
    %\tablecomments{$\sigma(\pi_{\rm E, \parallel}) \sim 0.05$}
    \label{parm6}
\end{table*}

==> table_backup.tex <==




For a lensing object, if both the angular Einstein radius, $\thetae$, and the microlensing parallax, $\pie$, are measured, the lens mass, $M_{\rm L}$, and the lens distance, $D_{\rm L}$, can be uniquely determined by the relations
\begin{equation}\label{eq:mass}
    M_{\rm L} = \frac{\thetae}{{\kappa}\pie};\qquad D_{\rm L} = \frac{\mathrm{au}}{\pie\thetae + \pi_{\rm S}},
\end{equation}
where $\kappa \equiv 4G/(c^2\mathrm{au}) = 8.144$ mas$/M_{\odot}$, $\pi_{\rm S} = \mathrm{au}/D_{\rm S}$ is the source parallax, and $D_{\rm S}$ is the source distance. However, for the present case neither $\thetae$ nor $\pie$ is unambiguously measured. Thus, we conduct a Bayesian analysis based on a Galactic model to estimate the lensing physical parameters. 

\begin{table*}
    \renewcommand\arraystretch{1.5}
    \centering
    \caption{Physical Parameters for 2L1S Models from a Bayesian Analysis}
    \begin{tabular}{c|c c c c c}
    \hline
    \hline
     Solution  & $M_{\rm host}[M_{\odot}]$ & $M_{\rm planet}[M_{\oplus}]$ & $D_{\rm L}$[kpc] & $a_{\bot}$[au] & $\mu_{\rm rel}$[${\rm mas\,yr^{-1}}$] & Gal.Mod. \\
    \hline
   
    A  & $0.50^{+0.38}_{-0.29}$ & $15.58^{+13.79}_{-9.27}$ & $7.53^{+0.87}_{-1.54}$ & $5.75^{+2.39}_{-2.00}$ & $3.17^{+1.55}_{-1.13}$ & 0.366 \\
    B & $0.28^{+0.34}_{-0.17}$ & $4.86^{+6.46}_{-3.02}$ & $7.67^{+0.77}_{-0.95}$ & $4.08^{+1.83}_{-1.30}$ & $6.83^{+3.26}_{-2.77}$ & 0.762 \\
    C & $0.37^{+0.36}_{-0.22}$ & $6.81^{+7.04}_{-4.11}$ & $7.64^{+0.79}_{-1.07}$ & $5.19^{+2.07}_{-1.59}$ & $5.44^{+2.54}_{-2.09}$ & 1.000 \\ 
    D & $0.67^{+0.37}_{-0.34}$ & $496.30^{+304.04}_{-260.76}$ & $6.47^{+1.21}_{-2.46}$ & $0.90^{+2.68}_{-2.38}$ & $7.25^{+2.52}_{-1.97}$ & 0.174 \\
    E & $0.47^{+0.34}_{-0.24}$ & $366.00^{+303.04}_{-188.15}$ & $0.80^{+1.08}_{-0.42}$ & $0.55^{+0.42}_{-0.26}$ & $15.78^{+13.98}_{-4.94}$ & 0.003 \\
    F & $0.64^{+0.36}_{-0.32}$ & $697.27^{+431.51}_{-356.17}$ & $6.95^{+0.96}_{-1.96}$ & $0.97^{+0.24}_{-0.23}$ & $6.62^{+2.50}_{-2.27}$ & 0.688 \\
    G & $0.51^{+0.44}_{-0.27}$ & $181.45^{+169.09}_{-94.03}$ & $2.22^{+1.93}_{-1.52}$ & $0.84^{+0.53}_{-0.43}$ & $12.93^{+4.55}_{-2.87}$ & 0.012 \\
    H & $0.66^{+0.39}_{-0.32}$ & $295.81^{+181.66}_{-143.45}$ & $3.86^{+1.66}_{-2.11}$ & $1.16^{+0.35}_{-0.47}$ & $7.88^{+3.95}_{-1.58}$ & 0.043 \\
    \hline
    \hline
    \end{tabular}\\
    \tablecomments{Gal.Mod. represents the relative probability from the Galactic model.}
    \label{phy}
\end{table*}


\begin{table*}
    \renewcommand\arraystretch{1.5}
    \centering
    \caption{$\theta_*$, $\thetae$ and $\mu_{\rm rel}$ for 2L1S xallarap Models}
    \begin{tabular}{c|c c c c c c c c}
    \hline
    \hline
    Model & A & B & C & D & E & F & G & H \\
    \hline
    $(V - I)_{\rm cl}$ & $2.09 \pm 0.01$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ \\
    $(V - I)_{\rm cl, 0}$ & $1.06 \pm 0.03$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ \\
    $I_{\rm cl}$ & $15.73 \pm 0.01$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ \\  
    $I_{\rm cl,0}$ & $14.49 \pm 0.04$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ \\
    $(V - I)_{\rm S}$  & $1.95 \pm 0.04$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ \\
    $(V - I)_{\rm S,0}$ & $0.92 \pm 0.05$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ & $\gets$ \\
    $I_{\rm S,0}$ & $16.11^{+0.50}_{-0.18}$ & $16.32^{+0.52}_{-0.23}$ & $16.46^{+0.44}_{-0.35}$ & $16.89^{+0.19}_{-0.22}$ & $16.72^{+0.24}_{-0.22}$ & $16.76^{+0.27}_{-0.25}$ & $16.96^{+0.17}_{-0.18}$ & $16.74^{+0.24}_{-0.22}$ \\
    $\theta_*$ ($\mu$as) & $2.33^{+0.23}_{-0.50}$ & $2.11^{+0.26}_{-0.47}$ & $1.91^{+0.35}_{-0.36}$ & $1.62^{+0.19}_{-0.16}$ & $1.76\pm0.20$ & $1.73 \pm 0.23$ & $1.57^{+0.15}_{-0.14}$ & $1.74\pm0.20$ \\
    $\thetae$ (mas)  & $>0.09$ & $>0.11$ & $>0.11$ & $>0.46$ & $>1.36$ & $>0.28$  & $>0.90$ & $>0.67$ \\ 
    $\mu_{\rm rel}$ (${\rm mas\,yr^{-1}}$) & $>0.72$ & $>1.2$ & $>1.2$ & $>6.0$ & $>12.4$ & $>3.3$ & $>10.4$ & $>6.2$ \\
    \hline
    \hline
    \end{tabular}
    \tablecomments{The lower limits for $\thetae$ and $\mu_{\rm rel}$ are at $3\sigma$.}
    \label{source}
\end{table*}




\textbf{OLD:}

    \begin{tabular}{c|c c c c c}
    \hline
    \hline
 & D  & E & F & G & H \\
\hline
$\chi^2$/dof & $ 10078.2/10682 $  & $ 10085.0/10682 $  & $ 10096.5/10682 $  & $ 10080.4/10682 $  & $ 10074.8/10682 $  \\
\hline
$t_0$ & $ 7881.23\pm0.87 $  & $ 7883.08^{+1.28}_{-1.93} $  & $ 7884.30^{+0.98}_{-1.47} $  & $ 7882.18\pm0.40 $  & $ 7881.81^{+2.17}_{-3.25} $  \\
$u_0$ & $ 1.053\pm0.074 $  & $ 1.13\pm0.15 $  & $ 1.26\pm0.15 $  & $ 1.218^{+0.037}_{-0.046} $  & $ 1.668\pm0.097 $  \\
$t_\mathrm{E}$ (days) & $ 27.92^{+1.38}_{-1.02} $  & $ 29.98^{+2.47}_{-1.86} $  & $ 31.25^{+2.80}_{-1.64} $  & $ 31.53\pm0.78 $  & $ 39.73\pm2.12 $  \\
$\rho$ ($10^{-2}$) & $ 0.041^{+0.048}_{-0.030} $  & $ 0.034^{+0.037}_{-0.024} $  & $ 0.336^{+0.086}_{-0.062} $  & $ 0.077\pm0.029 $  & $ 0.069^{+0.042}_{-0.035} $  \\
$t_{0,\mathrm{pl}}$ & $ 7810.326^{+0.058}_{-0.081} $  & $ 7810.307^{+0.054}_{-0.077} $  & $ 7810.05^{+0.11}_{-0.14} $  & $ 7810.380^{+0.035}_{-0.048} $  & $ 7810.225^{+0.057}_{-0.075} $  \\
$t_\mathrm{E,pl}$ & $ 1.35\pm0.13 $  & $ 1.47^{+0.21}_{-0.15} $  & $ 1.82^{+0.27}_{-0.19} $  & $ 1.052\pm0.093 $  & $ 1.48\pm0.12 $  \\
$\xi_P$ (days) & $ 100.3\pm5.4 $  & $ 174.4^{+20.1}_{-15.8} $  & $ 160.6\pm13.0 $  & $ 75.9^{+9.0}_{-6.2} $  & $ 146.5^{+14.3}_{-10.5} $  \\
$\xi_a$ & $ 0.227\pm0.059 $  & $ 0.37^{+0.12}_{-0.09} $  & $ 0.331^{+0.085}_{-0.069} $  & $ 0.048^{+0.013}_{-0.008} $  & $ 0.346\pm0.050 $  \\
$\xi_\Omega$ (deg) & $ 96.4^{+3.6}_{-2.6} $  & $ 132.7\pm6.7 $  & $ 312.5\pm8.0 $  & $ 292.9\pm10.0 $  & $ 134.6^{+7.2}_{-8.7} $  \\
$\xi_i$ (deg) & $ 117.1^{+2.6}_{-3.3} $  & $ 110.0\pm9.7 $  & $ 116.3\pm8.7 $  & $ 115.0^{+8.8}_{-11.5} $  & $ 128.1^{+2.9}_{-2.3} $  \\
$\xi_u$ (deg) & $ 75.5\pm13.6 $  & $ 120.8\pm16.0 $  & $ 282.8\pm12.6 $  & $ 162.4^{+31.3}_{-26.0} $  & $ 28.7\pm10.5 $  \\
$I_{\rm S}$ & $18.13^{+0.19}_{-0.22}$ & $17.96^{+0.24}_{-0.22}$ & $18.00^{+0.27}_{-0.25}$ & $18.20^{+0.17}_{-0.18}$ & $17.98^{+0.24}_{-0.22}$  \\
\hline
$s$ & $ 0.3266^{+0.0097}_{-0.0072} $  & $ 0.334^{+0.013}_{-0.009} $  & $ 0.333^{+0.016}_{-0.011} $  & $ 0.3427\pm0.0071 $  & $ 0.356^{+0.014}_{-0.011} $  \\
$q$ ($10^{-4}$) & $ 23.1^{+5.3}_{-4.0} $  & $ 23.9^{+4.6}_{-3.5} $  & $ 33.8^{+6.7}_{-5.5} $  & $ 11.1^{+2.7}_{-2.0} $  & $ 13.7\pm2.2 $  \\
$\alpha$ (deg) & $ 16.89\pm1.87 $  & $ 19.18\pm3.83 $  & $ 21.19\pm3.74 $  & $ 32.30\pm0.45 $  & $ 47.57^{+3.26}_{-2.49} $  \\
\hline\hline
\end{tabular}
\label{tab:2L1S_xa2}

\textbf{NEW:}




\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{Lensing Parameters for 2L2S Static Models}
    \begin{tabular}{c|c c c}
    \hline
    \hline
     Parameters & Close Upper & Close Lower & Wide \\
    \hline
    $\chi^2$/dof & $16137.3/10683$ & $16100.9/16083$ & $16096.5/16083$  \\
    \hline
    $t_{0,1}$ (${\rm HJD}^{\prime}$)  & $7888.233 \pm 0.941$ & $7883.734 \pm 0.644$ & $\mathbf{7889.776 \pm 1.325}$  \\
    $t_{0,2}$ (${\rm HJD}^{\prime}$) & $7867.483 \pm 0.867$ & $7864.920 \pm 1.021$  & $\mathbf{7868.363 \pm 0.963}$  \\
    $u_{0,1}$  & $1.5187 \pm 0.0128$ & $1.4768 \pm 0.0118$ & $\mathbf{1.5211 \pm 0.0138}$  \\
    $u_{0,2}$ & $0.9971 \pm 0.0545$ & $0.7199 \pm 0.0899 $ &  $\mathbf{1.0729 \pm 0.0533}$ \\
    $\te$ (days)  & $27.24 \pm 0.26$ & $28.57 \pm 0.22$ & $\mathbf{27.02 \pm 0.26}$  \\
    $\rho$ ($10^{-2}$)  & $0.238 \pm 0.066$ & $<0.120\ (3\sigma)$ & $\mathbf{<0.765\ (3\sigma)}$  \\
    $q_{f,I} $ & $0.2305 \pm 0.0498$ & $0.0533 \pm 0.0157$ & $\mathbf{0.3455 \pm 0.1307}$  \\
    $\alpha$ (rad)  & $0.3680 \pm 0.0142$ & $0.5993 \pm 0.0054$ & $\mathbf{3.5883 \pm 0.0558}$  \\
    $s$ & $0.285 \pm 0.004$ & $0.307 \pm 0.003$ & $\mathbf{3.588 \pm 0.056}$  \\
    $q (10^{-4})$ &$34.364 \pm 5.257$ &$12.833 \pm 1.150$ & $\mathbf{0.692 \pm 0.093}$\\
    $\log q$ & $-2.464 \pm 0.066$ & $-2.892 \pm 0.039$ & $\mathbf{-4.160 \pm 0.058}$  \\
    $f_{\rm S, OGLE}$ & $2.82930 \pm 0.00011$ & $2.82919 \pm 0.00013$ & $\mathbf{2.82925 \pm 0.00018}$  \\
    %f_{\rm B, OGLE}$ & $0$ & $\mathbf{0}$ & $0$ & $0$ \\
    \hline
    \hline
    \end{tabular}
    \tablecomments{Fix $f_{\rm B, OGLE} = 0$. All fluxes are on an 18th magnitude scale, e.g., $I_{\rm S} = 18 - 2.5 \log(f_{\rm S})$. Fix the second source's radius at $10^{-3}$.}
    \label{parm3}
\end{table*}



\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{Lensing Parameters for 2L2S Parallax Models}
    \begin{tabular}{c|c c |c c| c c}
    \hline
    \hline
    Parameters & \multicolumn{2}{c|}{Close Upper} & \multicolumn{2}{c|}{Close Lower} & \multicolumn{2}{c}{Wide} \\
    %\hline
     & $u_{0,1} > 0$ & $u_{0,1} < 0$ & $u_{0,1} > 0$ & $u_{0,1} < 0$ & $u_{0,1} > 0$ & $u_{0,1} < 0$ \\
    \hline
    $\chi^2$/dof & $16127.3/16081$ & $16114.0/16081$ & $16097.7/16081$ & $16137.3/16081$ & $16088.3/16081$ & $16088.1/16081$ \\
    \hline
    $t_{0,1}$ (${\rm HJD}^{\prime}$)  & $7880.385 \pm 3.136$ & $78803.177 \pm 3.280$ & $7879.627 \pm 2.061$ & $7886.795 \pm 1.281$ & $7881.153 \pm 3.310$ & $7879.339 \pm 3.686$ \\
    $t_{0,2}$ (${\rm HJD}^{\prime}$)  & $7863.217 \pm 1.776$  & $7864.752 \pm 1.867$ & $7863.590 \pm 1.198$  & $7861.753 \pm 1.232$ & $7864.469 \pm 1.818$ & $7867.788 \pm 1.905$  \\
    $u_{0,1}$  & $1.5014 \pm 0.0579$ & $-1.4755 \pm 0.0690$ & $1.5799 \pm 0.0406$ & $-1.3300 \pm 0.0473$ & $1.6315 \pm 0.0776$ & $-1.6106 \pm 0.0609$ \\
    $u_{0,2}$  & $0.9973 \pm 0.0597 $ &  $1.0444 \pm 0.0747$ & $0.9135 \pm 0.0969 $ &  $0.8601 \pm 0.0513$ & $1.2415 \pm 0.0827$ & $1.1583 \pm 0.0594$ \\
    $\te$ (days)  & $24.70 \pm 0.94$ & $25.60 \pm 0.96$ & $26.62 \pm 0.78$ & $27.79 \pm 0.34$ & $24.19 \pm 1.11$ & $23.82 \pm 1.18$  \\
    $\rho$ ($10^{-2}$)  & $0.403 \pm 0.079$ & $0.226 \pm 0.035$ & $<0.125\ (3\sigma)$ & $<0.395\ (3\sigma)$ & $<0.372\ (3\sigma)$ & $<0.831\ (3\sigma)$ \\
    $q_{f,I} $ & $0.1637 \pm 0.0457$ & $0.2184 \pm 0.1093$ & $0.0960 \pm 0.0210$ & $0.0735 \pm 0.0149$ & $0.4806 \pm 0.1136$ & $0.5901 \pm 0.1579$  \\
    $\alpha$ (rad)  & $0.3596 \pm 0.0231$ & $5.6894 \pm 0.0274$ & $0.6324 \pm 0.0139$ & $5.9192 \pm 0.0151$ & $3.6523 \pm 0.0238$ & $2.6318 \pm 0.0203$  \\
    $s$  & $0.287 \pm 0.002$ & $0.287 \pm 0.005$ & $0.300 \pm 0.003$ & $0.299 \pm 0.002$ & $3.627 \pm 0.048$ & $3.593 \pm 0.045$  \\
    $q (10^{-4})$ &$38.345 \pm 4.965$ & $29.469 \pm 8.075$ &$16.225 \pm 1.623$ & $19.697 \pm 3.185$ &$0.983 \pm 0.180$ & $1.074 \pm 0.212$ \\
    $\log q$ & $-2.416 \pm 0.056$ & $-2.531 \pm 0.119$ & $-2.790 \pm 0.043$ & $-2.752 \pm 0.078$ & $-4.007 \pm 0.079 $ & $-3.969 \pm 0.086$ \\
    $\pi_{\rm E, N}$ & $0.015 \pm 0.065$ & $0.014 \pm 0.087$ & $0.109 \pm 0.043$ & $0.184 \pm 0.052$ & $0.136 \pm 0.084$ & $-0.186 \pm 0.088$ \\
    $\pi_{\rm E, E}$  & $0.218 \pm 0.074$ & $0.159 \pm 0.076$ & $0.107 \pm 0.048$ & $0.095 \pm 0.036$ & $0.231 \pm 0.091$ & $0.272 \pm 0.100$  \\
    $f_{\rm S, OGLE}$  & $2.82928 \pm 0.00013$ & $2.82916 \pm 0.00012$ & $2.82933 \pm 0.00013$ & $2.82913 \pm 0.00014$ & $2.82933 \pm 0.0019$ & $2.82932 \pm 0.00024$ \\
    %f_{\rm B, OGLE}$ & $0$ & $\mathbf{0}$ & $0$ & $0$ \\
    \hline
    \hline
    \end{tabular}
    \tablecomments{Fix $f_{\rm B, OGLE} = 0$. All fluxes are on an 18th magnitude scale, e.g., $I_{\rm S} = 18 - 2.5 \log(f_{\rm S})$. Fix the second source's radius at $10^{-3}$.}
    \label{parm4}
\end{table*}

\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{Lensing Parameters for 1L2S Models}
    \begin{tabular}{c|c| c c}
    \hline
    \hline
    Parameters & Static & \multicolumn{2}{c}{Parallax}  \\
     & & $u_{0,1}>0$ & $u_{0,1}<0$ \\
    \hline
    $\chi^2$/dof & $16375.3/16086$ & $16105.8/16084$ & $16159.1/16084$ \\
    \hline
    $t_{0,1}$ (${\rm HJD}^{\prime}$)  & $7879.997 \pm 0.088$ & $7852.702 \pm 7.426$ & $7861.924 \pm 5.841$ \\
    $t_{0,2}$  & $7810.605 \pm 0.004$ & $7810.598 \pm 0.008$ & $7810.601 \pm 0.006$ \\
    $u_{0,1}$  & $1.4093 \pm 0.0041$ & $1.8528 \pm 0.1486$ & $-1.6925 \pm 0.2278$ \\
    $u_{0,2}$  & $0.00156 \pm 0.00022$ & $0.00369 \pm 0.00128$ & $0.00227 \pm 0.00028$ \\
    $\te$ (days)  & $29.16 \pm 0.12$ & $16.25 \pm 3.30$ & $20.88 \pm 1.72$ \\
    $\rho$  & $< 0.240\ (3\sigma)$ & $< 0.361\ (3\sigma)$ & $< 0.216\ (3\sigma)$ \\
    $q_{f,I}(10^{-3})$  & $0.392 \pm 0.260$ & $1.110 \pm 0.185$ & $0.751 \pm 0.313$ \\
    $\pi_{\rm E, N}$  & ... & $0.81 \pm 0.26$ & $-0.47 \pm 0.31$ \\
    $\pi_{\rm E, E}$  & ... & $1.43 \pm 0.35$ & $0.67 \pm 0.12$ \\
    $f_{\rm S, OGLE}$ & $2.82943 \pm 0.00012$ & $2.82933 \pm 0.00016$ & $2.82902 \pm 0.00011$ \\
    %f_{\rm B, OGLE}$ & $0$ & $\mathbf{0}$ & $0$ & $0$ \\
    \hline
    \hline
    \end{tabular}
    \tablecomments{Fix $f_{\rm B, OGLE} = 0$. All fluxes are on an 18th magnitude scale, e.g., $I_{\rm S} = 18 - 2.5 \log(f_{\rm S})$.}
    \label{parm5}
\end{table*}






%\begin{table}
%    \renewcommand\arraystretch{1.5}
%    \centering
%    \caption{CMD parameters, $\theta_*$, $\thetae$ and $\mu_{\rm rel}$ for \evente}
%    \begin{tabular}{c|c c c }
%    \hline
%    \hline
%    Parameter & Close A & Close B & Wide  \\
%    \hline
%    $(V - I)_{\rm cl}$ & $2.89 \pm 0.01$ & $\gets$ & $\gets$ \\
%    $I_{\rm cl}$ & $16.42 \pm 0.02$ & $\gets$ & $\gets$  \\
%    $I_{\rm cl,0}$ & $14.33 \pm 0.04$ & $\gets$ & $\gets$ \\
%    $(V - I)_{\rm S}$ & $2.66 \pm 0.03$ & $\gets$ & $\gets$ \\
%    $I_{\rm S}$ & $21.26 \pm 0.06$ & $21.19 \pm 0.08$ & $21.22 \pm 0.06$ \\
%    $(V - I)_{\rm S,0}$ & $0.83 \pm 0.04$ & $\gets$ & $\gets$ \\
%    $I_{\rm S,0}$ & $19.17 \pm 0.07$ & $19.10 \pm 0.09$ & $19.13 \pm 0.07$ \\
%    $\theta_*$ ($\mu$as) & $0.526 \pm 0.027$ & $0.543 \pm 0.032$ & $0.540 \pm 0.028$ \\
%    $\thetae$ (mas)  & $0.453 \pm 0.142$ & $0.267 \pm 0.084$ & $>0.42$ \\ 
%    $\mu_{\rm rel}$ (${\rm mas\,yr^{-1}}$) & $2.17 \pm 0.68$ & $1.35 \pm 0.42$ & $>2.1$ \\
%    \hline
%    \hline
%    \end{tabular}
%    \tablecomments{$(V - I, I)_{\rm cl,0} = 1.06 \pm 0.03$}
%    \label{source2}
%\end{table}





%\begin{table}
%    \renewcommand\arraystretch{1.5}
%    \centering
%    \caption{Preliminary physical parameters of the lens systems, inferred from the Bayesian analysis.}
 %   \begin{tabular}{c c c}
 %   \hline
 %   \hline
 %    & $I_{\rm L} > 20$ & $I_{\rm L} > 21$ \\
 %   \hline
 %   $M_{\rm host}[M_{\odot}]$ & $0.59_{-0.22}^{+0.21}$ & $0.51_{-0.18}^{+0.15}$ \\
    
%    $M_{\rm planet} [M_\oplus]$ & $1.18_{-0.57}^{+1.00}$ & $1.01_{-0.48}^{+0.83}$ \\
    
 %   $D_{\rm L}$[kpc] & $6.27_{-1.69}^{+0.78}$ & $6.44_{-1.80}^{+0.71}$ \\
    
 %   $a_{\perp}$[au] & $2.88_{-0.68}^{+0.58}$ & $2.65_{-0.62}^{+0.46}$ \\
    
 %   $\mu_{\rm rel}$[${\rm mas\,yr^{-1}}$] & $1.25_{-0.36}^{+0.46}$ & $1.11_{-0.30}^{+0.40}$ \\
 %   \hline
 %   \hline
 %   \end{tabular}\\
    %\tablecomments{The inferred parameters }
 %   \label{phy}
%\end{table}











\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{Lensing Parameters for 3L1S Static Models}
    \begin{tabular}{c|c  c  c}
    \hline
    \hline
    Parameters & Close Upper & Close Lower & Wide \\
    \hline
    $\chi^2$/dof & $16130.0/16083$ & $16091.4/16083$ &  $16088.8/16083$ \\
    \hline
    $t_{0}$ (${\rm HJD}^{\prime}$)  & $7884.617 \pm 0.316$  & $7884.219 \pm 0.165$ & $7884.285 \pm 0.412$\\
    $u_{0}$  & $1.4690 \pm 0.0060$  & $1.4658 \pm 0.0060$ & $1.4650 \pm 0.0071$\\
    $\te$ (days)  &  $29.216 \pm 0.219$ & $29.897 \pm 0.204$  & $29.564 \pm 0.274$\\
    $\rho$ ($10^{-2}$)  &  $0.284 \pm 0.578$  & $<0.046\ (3\sigma)$ & $1.360 \pm 0.116$\\
    $\alpha$ (rad)  &  $5.9287 \pm 0.0544$  & $5.8814 \pm 0.0106$& $5.8835 \pm 0.0872$\\
    $s_2$ & $0.318 \pm 0.004$  & $0.308 \pm 0.004$& $0.311 \pm 0.004$\\
    $q_2 (10^{-1})$ & $7.081 \pm 0.927$  & $8.668 \pm 0.399$& $8.457 \pm 1.704$\\
    $\log q_2$ & $-0.150 \pm 0.057$  & $-0.062 \pm 0.020$& $-0.073 \pm 0.087$\\
    $s_3$ & $0.456 \pm 0.004$  & $0.430 \pm 0.004$& $3.1305 \pm 0.023$\\
    $q_3 (10^{-4})$ & $38.996 \pm 5.629$  & $20.650 \pm 2.420$& $0.955 \pm 0.287$\\
    $\log q_3$ & $-2.409 \pm 0.063$  & $-2.685 \pm 0.051$& $-4.020 \pm 0.131$\\
    $\psi$ (rad) & $5.9261 \pm 0.0273$  & $5.7771 \pm 0.0063$& $2.1715 \pm 0.0892$\\
    $f_{\rm S, OGLE}$ & $2.82945 \pm 0.00013$  & $2.82936 \pm 0.00014$& $2.82922 \pm 0.00012$\\
    \hline
    \hline
    \end{tabular}
    % \tablecomments{Fix $f_{\rm B, OGLE} = 0$. All fluxes are on an 18th magnitude scale, e.g., $I_{\rm S} = 18 - 2.5 \log(f_{\rm S})$.}
    % $\rho$ ($10^{-3}$)  &  $3.471 \pm 0.380$  & $<0.978 (3\sigma)$ & $13.05 \pm 0.62$\\
    \label{parm3L1S}
\end{table*}





\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{$\chi^2$ for different models}
    \begin{tabular}{c|c|c c c|c c c|c c c}
    \hline
    \hline
    $\chi^2$/dof & 1L1S &  & 2L1S &  &  & 2L2S &  &  & 3L1S &  \\
     &   & close upper & close lower & wide & close upper & close lower & wide & close upper & close lower & wide \\
    static & 17750 & 16338 & 16256 & 16292 & 16137 & 16101 & 16097  & 16130 & 16091 & 16089 \\
    parallax & 17661 & 16141 & 16113 & 16091 & 16114 & 16098 & 16088 & & &\\
    \hline
    \hline
    \end{tabular}
\end{table*}



